Selecting Data to Clean for Fact Checking: Minimizing Uncertainty vs. Maximizing Surprise

We study the optimization problem of selecting numerical quantities to clean in order to fact-check claims based on such data. Oftentimes, such claims are technically correct, but they can still mislead for two reasons. First, data may contain uncertainty and errors. Second, data can be "fished" to advance particular positions. In practice, fact-checkers cannot afford to clean all data and must choose to clean what "matters the most" to checking a claim. We explore alternative definitions of what "matters the most": one is to ascertain claim qualities (by minimizing uncertainty in these measures), while an alternative is just to counter the claim (by maximizing the probability of finding a counterargument). We show whether the two objectives align with each other, with important implications on when fact-checkers should exercise care in selective data cleaning, to avoid potential bias introduced by their desire to counter claims. We develop efficient algorithms for solving the various variants of the optimization problem, showing significant improvements over naive solutions. The problem is particularly challenging because the objectives in the fact-checking context are complex, non-linear functions over data. We obtain results that generalize to a large class of functions, with potential applications beyond fact-checking.

==> expr-old/expr.tex <==
\section{Experiments}
\label{sec:expr}
\subsection{Fairness}
In this section we run experiments on synthetic and real data using different algorithms
to reduce the uncertainty on Fairness.

\input{ExperimentsFairness.tex}

\paragraph{Data}
We consider Giuliani's claims. This real dataset consists of the number of adoptions in NYC
from 1989-2014. For each year we have a tuple whose value represents the number of adoptions
in this year. In order to generate uncertainty, we consider a normal distribution
for each tuple. For a tuple $t_i$, the expected value $M_i$ is the reported number of adoptions of that year,
and the standard deviation is a random number in $[1,50]$. Each tuple has also a deterministic
cost that we generated as a uniform random sample in $[1,100]$.

The structure of the claims is the following. Each claim consists of two, four
year periods of time. For example $c_1$ would consist of the periods $[1,4]$, $[5,8]$
that correspond to the periods $[1989-1992]$, $[1993-1996]$.
The value of claim $c_1$ is defined as $Val[c_1] = D_5+D_6+D_7+D_8 - (D_1+D_2+D_3+D_4)$.
Equivalently we can define the value for all claims $c_j$. In total, we have $19$ claims.
The sensibility of the claims is generated as follows. We consider an Exponential
distribution with $\lambda=1.5$. We take $19$ random numbers in the range $[0,5]$,
and for each number we find the probability density of the exponential
distribution with $\lambda=1.5$. Then, we sort the results in increasing order and
we assign the sensibilities to the claims following the sorted order, i.e.
claims back in time will have less sensibility than recent claims.
We call the dataset $Std50Cost100Exp$. With the same way we can generate other
datasets, $StdXCostYZ$, where $X$ is the upper bound on the standard deviation
of the normal distributions, $Y$ is the upper bound of the cleaning cost, and $Z$
is the distribution that we use to generate the sensibilities.

\input{AllUniform.tex}

\paragraph{Algorithms}
\begin{enumerate}
 \item \OptF{}: We implement the pseudo-polynomial algorithm using DP
 for Knapsack problem and use it to find the optimum set of tuples to clean to reduce
 the variance.
 \item \GreedyF{}: The simple greedy algorithm for the Knapsack problem:
 Using the notation of $P_2$, we sort in increasing order the ratios $\frac{a_i}{b_i}$
 and start cleaning the tuples following that order.
 \item \BlindF{}: Similar to \GreedyF{} but we sort the tuples only
 with respect to $a_i$'s.
 \item \RandomF{}: An algorithm that chooses every time the next tuple to clean
 uniformly at random.
\end{enumerate}

In Figure \ref{fig:ExpFairness} we can see the efficiency of all algorithms in $Std50Cost100Exp$.
\RandomF{} algorithm is the worst comparing with the other algorithms
so we will not consider it in our analysis. In all cases \OptF{} is obviously
the best algorithm. \GreedyF{} algorithm is also very efficient and close to the
optimum solution of the algorithm. On the other hand a simpler greedy algorithm,
\BlindF{} does not perform very efficiently in all executions. In Figure \ref{fig:ExpFairness} (right)
we show the results for a subset of the budget. Clearly, from budget $90$ to $270$
\BlindF{} cannot reduce the uncertainty of the Fairness by a lot.


Notice that, it is easy to generate synthetic data such that \BlindF{}
is much worse than the other algorithms at least for a subset of the budget. That
is because, to reduce the variance in Fairness we actually solve a Knapsack problem
and in the worst case the approximation ratio of the \BlindF{} is unbounded.
Similarly, we can have synthetic cases where the greedy algorithm is twice as bad as the
optimum one, at least for a subset of the budgets.

\subsection{Uniqueness}

In this subsection we run experiments on synthetic data using different algorithms
to reduce the expected variance on Uniqueness.

\input{LogNormal.tex}

\paragraph{Data}
We show results for five different random and synthetic datasets. Overall, we consider
$m=10$ independent claims and $n=40$ tuples with $w=4$.
In each dataset we generate the distribution and the cleaning cost of each tuple with different ways.
\begin{itemize}
  %\item AllUniform: Each tuple has a discrete distribution that takes four different values: $1, 2, 3, 4$ with probabilities $p_1, p_2, p_3, p_4$. For each tuple,
  %it holds that $p_1+p_2+p_3+p_4=1$. The probabilities $p_i$ are generated uniformly at random. The cleaning cost of each tuple is also generated uniformly at
  %random in the range $[1,10]$. Notice that the value of each claim is the range $[4, 12]$. We show the results for $r_0= 4, 8, 10$.
  \item AllUniform: Each tuple has a discrete distribution that takes at least one and at most six different values. Each value is chosen uniformly at random in the range $[1,100]$, and the probabilities are also uniform number is $[0,1]$. The cleaning cost of each tuple is generated uniformly at
  random in the range $[1,10]$. Notice that the value of each claim is the range $[0, 400]$.
  %\item UniformCost1: Same with AllUniform, but the cleaning cost of each tuple is $1$. We show the results for $r_0= 4, 8, 10$.
%  \item NonUniformCost1: Almost the same with UniformCost1. For each value, the probability of the discrete distribution is either very small or very large.
%  We show the results for $r_0=4, 8, 10$.
%  \item NonUniformProbs\_NonUniformCosts: The cost of each tuple is $1$ with probability $1/2$, or $10$ otherwise. The probabilities are given as in %NonUniformCost1.
 % We show the results for $r_0= 4, 8, 10$.
 \item LogNormalProbs\_UniCosts: The cost of each tuple is chosen uniformly at random in the range $[1,10]$.
 %For each tuple, we create a distribution by discretizing a LogNormal distribution.
 For each tuple, we first generate the LogNormal distribution with parameters $(0,r)$, where $r$ is a random
 number between $0$ and $1$. To create the tuples's distribution, we discretize the LogNormal distribution using at most $6$ discrete points.
  \item NonUniProbs\_UniCosts: The cost of each tuple is chosen uniformly at random in the range $[1,10]$. The discrete distribution for the value
  of a tuple takes at least one and at most six possible values. The values are uniform numbers in the range $[1,100]$. For each value distribution, we assign the probabilities, such that some probabilities are very tiny and the rest are large.
  \item UniProbs\_NonUniCosts: The cost of each tuple is $1$ with probability $1/2$, or $10$ otherwise. The discrete distribution for the value
  of a tuple takes at least one and at most six possible values. The values are uniform numbers in the range $[1,100]$. For each value distribution, we assign
  probabilities chosen uniformly at random.
\end{itemize}

\input{UniProbsnonUniCosts.tex}

\paragraph{Algorithms}
We implement two algorithms to compare their efficiency on reducing the uncertainty
on Uniqueness.
\begin{enumerate}
 \item \BestU{}: We implemented the approximation algorithm \cite{iyer2013submodular} with theoretical guarantees
 described in the Uniqueness section above.
 \item \GreedyU{}: The greedy algorithm for the \MinVar\ problem.
 \item \NaiveU{}: This is the naive greedy algorithm for the \MinVar\ problem.
 %We compute and sort in decreasing order the ratios $\frac{V_i}{b_i}$: We clean tuples following the decreasing order until we exceed the budget $b$.
\end{enumerate}


Our goal is to reduce the $\EVar{}$ of the following function $\sum_{j=1}^m \One{X_{j1}+\ldots+X_{jW}<r_0}$, where claim $j$
contains the objects $X_{j1}, \ldots, X_{jW}$. For simplicity we consider independent claims.
Before presenting the results notice that the uncertainty of a claim highly depends on the value of $r_0$.
Hence, we try different values of $r_0$ and show the behavior of the studied algorithms.


Given an $r_0$, for each data set we show the $\EVar$ achieved by all the algorithms for all possible given budgets.
For each figure that we present, the $x$ axis represents the budget and the $y$ axis represents the value of the $\EVar{}$.
In Figures~\ref{fig:AllU}, \ref{fig:Log}, \ref{fig:nonUniProbsUniCosts}, \ref{fig:UniProbsnonUniCosts}, we show the results for all datasets.
In all cases, Best and GreedyMinVar are the best algorithm. The simpler NaiveGreedy algorithm cannot reduce the uncertainty
of the claims by much.

\input{nonUniProbsUniCosts.tex}

We focus on AllUniform data set.
When the value $r_0$ is around $200$, the uncertainty is too large. For example, note that the variance before starting cleaning any object
is more than $1.6$ compared to the expected variance of $0.45$ for $r_0=100$. The relative difference in the efficacy of the algorithms
seems smaller as $r_0$ takes values that maximize the initial uncertainty. In other words, it seems that all algorithms
perform almost the same when $r_0=200$. This is also the case for NonUniProbs\_UniCosts and UniProbs\_NonUniCosts data sets for $r_0=200$.
(For the LognNormal data set is not too clear what value of $r_0$ gives the maximum initial uncertainty).


In contrast, we observe that as the initial uncertainty becomes higher, the absolute difference in $\EVar{}$ between the algorithms
is not tiny. We show the results for LogNormal data set but the same results hold for the other data sets as well.
The $x$-axis of Figure~\ref{fig:DifLog} represents the budget, while the $y$-axis is the absolute difference between the $\EVar$ returned
by the \GreedyNaive{} and \Greedy{} algorithm. From Figures ~\ref{fig:DifLog}, \ref{fig:Log} we see that the absolute difference
between the two algorithms is higher when $r_0=4$, which is also the value with the highest initial uncertainty.
The difference is also high when $r_0=3.5$ or $r_0=4.5$, i.e. values that give high initial uncertainty as well.
For $r_0=3$, \Greedy{} seem to perform much  better than \GreedyNaive{} algorithm in Figure~\ref{fig:Log},
however the absolute difference between the algorithms is tiny.
Furthermore, as we expected, the difference between \Greedy{} (or \OPT{}) and \GreedyNaive{} is increasing as the budget increases until some budget $b$,
and then the difference is decreasing as the budget further increases.

\input{DifAllUniform.tex}

Overall, we do not observe many difference between \OPT{} and \Greedy{} algorithm. This is intuitive since the approximation factor of \OPT{} algorithm
depends on the curvature of the objective function which may be large. However, in any case, both \OPT{} and \Greedy{} perform much better than \GreedyNaive{} algorithm.


\paragraph{Efficiency}
Previously, we show that \OPT{} and \Greedy{} reduce the uncertainty by a much larger amount comparing to the \GreedyNaive{} algorithm.
Here, we measure the running time of our proposed algorithms. We focus only on the running time of \Greedy{} because it performs
very similar to \OPT{} and it is generally much faster than it. The \GreedyNaive{} algorithm does not use the objective function
and from its implementation it is very fast. Ideally, we want a reasonable running time for \Greedy{}.
In Figure~\ref{fig:Time} we show the scalability of \Greedy{} through two plots.
For the first one, we generate $10000$ tuples as in the AllUniform data set, i.e., all values are chosen uniformly at random.
We test the running time in seconds for different budgets. In particular, we try budgets equal to $1\%, 5\%, 10\%, 20\%, 30\%$ of the
maximum possible budget, which is defined as the sum of weights of all tuples, $\sum_{i=1}^n c_i$.
Intuitively, as the budget increases the running time also increases, however we always get a result not more than a couple of minutes.
For the second (right) plot of Figure~\ref{fig:Time} we fix the budget to be $\frac{10}{100}\sum_{i=1}^n c_i$, and we check the scalability
as the number of tuples increases. The running time is $0.031, 0.47, 48, 4521$ seconds for $n=100, 1000, 10000, 100000$, respectively.
We observe that \Greedy{} is very fast for a small number of tuples, and it requires a few or several minutes for larger number of tuples.

Overall, we conclude that \GreedyNaive{} is a very fast algorithm that returns a poor solution in terms of minimizing the variance of a function.
If we want to improve the results and decrease the uncertainty on claims' quality by a large amount, then we spend a few more minutes running \Greedy{} algorithm.

\input{Time.tex}




\subsection{Comparison between different objectives}
In the end of Section~\ref{sec:model}, we discussed how the objectives of
ascertaining the claim quality (fairness) vs increasing the chance of finding counterarguments
can be different or equal depending on the current values $\*u$.
Here, we run some experiments on real data showing how different the results can be between
the two objectives.

In order to show the different goals of each problem and the need of different techniques
for each case, we run experiments on simplified Giuliani's claims. Each claim
$c_j$ consists of $W=4$ consecutive tuples \footnote{Without loss of generality, we do not consider
claims that are defined over two consecutive groups of tuples as we did in the previous experiments.}.
As we had before, the weight of a tuple is a Normal random variable with mean the reported number of adoptions
in the year, standard deviation is generated uniformly at random in $[1,50]$, the
cost is also generated uniformly at random in $[1,100]$ and the sensibility is generated
by sampling from Normal distribution.

To get a current value $\*u_i$, we sample from distribution $X_i$.

We present the results in Figure~\ref{fig:Compare}.
For a given budget $C$, we find the optimum set of objects to clean to reduce the variance on Fairness
running the dynamic programming algorithm for the Knapsack problem. Let $T^*$ be the optimum set of objects.
Using $T^*$, we find the value of the objective function for \MaxPr\, i.e. the probability that in average a good counter claim exists.
We can see this probability with the blue color in Figure~\ref{fig:Compare} (right).
Then, we find a feasible solution for the \MaxPr\ to compare.
Since we do not have a method to solve it optimally,
we run a simple greedy algorithm to find a lower bound of its maximum probability, red color in Figure~\ref{fig:Compare} (right).
Since the results depend a lot on the current values, we sample $100$ times and we show the average.
As we can see, the probability that a good counter claim exists using Fairness' objective is much lower
than the probability that we get solving the \MaxPr\ problem.

Similarly, we get a solution for the \MaxPr\ problem, say $T_P^*$, and we compare the efficacy of $T_P^*$ to reduce the variance,
with the variance that we get if we solve the \MinVar\ problem straightforwardly. Again, as we can see in Figure~\ref{fig:Compare} (left) the
straightforward method of reducing the variance works much better than the method of maximizing the probability.

Hence, each objective function is different and different techniques should be used to optimize them.

\input{Fairness.tex}
%\input{Probs.tex} 

==> factcheck.tex <==
\section{Reduce the uncertainty on claims}
In this section we apply the results proved in the previous sections to some applications on Computational Journalism.
We use the framework proposed in \cite{wu2014toward}.
Database research has in the past focused on how
to answer queries, but has not devoted much attention to discerning more subtle qualities of the resulting claims, e.g.,
is a claim “cherry-picking”?
They model the problem of measuring the quality of a claim as an optimization problem for
\emph{Window Aggregate Comparison Claims} and \emph{Time Series Similarity Claims} that cover a broad area
of claims in practise. The key insight is that we can learn a lot about a claim by perturbing its parameters
and seeing how its conclusion changes, i.e. does a claim become stronger or weaker by changing its parameters?

Nowadays, because of data integration, pervasive computing, and scientific data analysis a lot of data are accompanied
with uncertainty. When dealing with uncertain data the computation of high quality claims becomes more challenging.
In this section, using the fact checking framework proposed in \cite{wu2014toward}, in presence of uncertainty,
we study the the problem of reducing the uncertainty on claims' quality and the problem of finding good \emph{counter claims}
as data cleaning problems.

Let $T=\{t_1,\ldots, t_n\}$ be a set of $n$ tuples and $C=\{c_1,\ldots, c_m\}$ a set of $m$ claims. Each claim is represented as a set of $w$ tuples in $T$.
In \cite{wu2014toward}, each tuple $t_i$ is associated with a value which is a non-negative discrete random variable $X_i$ with support $f$.
Furthermore, each tuple $t_i$ has a \emph{current value} $a_i\in \Re$.
Given a deterministic claim $c_0$ (random claim $c_0$ will not make any difference to the analysis so we keep it simple) with value $v_0$,
the sensibility $S(c_j,c_0)\in \Re$ denotes the relationship between claims $c_j, c_0$. If $S(c_j,c_0)$ is large then $c_j$ is closely
related with $c_0$, while if $S(c_j,c_0)$ is small then $c_j$ does not have a strong relationship with $c_0$.
By normalizing the sensibilities we can consider that they define a distribution over the claims, i.e. $\sum_{1\leq j\leq m}S(c_j,c_0)=1$,
and $0\leq S(c_j,c_0)\leq 1$.

Here, we concentrate on the Window Aggregate Comparison Claims but all the results hold for
Time Series Similarity Claims, as well. Given a reference claim $c_0$, the strength of a claim $c_j\in C$ is defined
as $V(c_j,c_0)=\sum_{t_i\in c_j}X_i-r_0$, where $r_0\in \Re$ is the deterministic value of claim $c_0$.
If $V(c_j,c_0)<0$, claim $c_j$ is weaker than claim $c_0$.
If $V(c_j,c_0)>0$, claim $c_j$ is stronger than $c_0$.

In \cite{wu2014toward}, they define some ways to measure the quality of claims.
Given a claim $c_0$ with value $r_0\in \Re$, they define:
\begin{itemize}
\item Fairness: $F(c_0)=\sum_{1\leq j\leq m} S(c_j,c_0)\cdot V(c_j,c_0)$
\item Uniqueness: $U(c_0)=\frac{1}{\cardin{C}}\cdot \sum_{1\leq j\leq m} \mathbbm{1}(V(c_j,c_0)<0)$
\item Robustness: $R(c_0)=\exp\left( -\sum_{1\leq j\leq m}S(c_j,c_0)\cdot (\min\{0, V(c_j,c_0)\})^2 \right)$
\end{itemize}
Intuitively, fairness is the expected strength of a perturbed claim generated by the random fact-
checker.  Fairness of $0$ means the claim is unbiased; positive fairness means the claim is understated; negative
fairness means it is overstated.
Uniqueness is the fraction of all possible parameter settings
that yield results weaker than the original claim. This definition does not require a parameter sensibility relation
or function. Low uniqueness means it is easy to find perturbed claims that are at least as strong as the original one.

Next, we define the data cleaning problems that arising, considering uncertainty on the values of the tuples.
For the next problems we also assume that each tuple has a cleaning cost $b_i\in \Re$. Given a budget
$b\in \Re$, the goal is to clean some tuples with cost at most $b$, to minimize the uncertainty on the measurements of the quality of the claims.

\subsection{Reduce Uncertainty on Fairness}
Our goal is to minimize the variance of Fairness measurement. Specifically, we want to choose a subset $A\subseteq T$ to clean such that:
\[
\min_{A\subseteq T, \sum_{t_i\in A} b_i\leq b} \Var{F(c_0)\mid \text{ Tuples }A\text{ are cleaned}}
\]
We can write the variance of $F(c_0)$ as,
\[
\Var{F(c_0)}=\Var{\sum_{1\leq j\leq m} S(c_j,c_0)\cdot V(c_j,c_0)}=\Var{\sum_{1\leq j\leq m} S(c_j,c_0)\sum{t_i\in c_j}X_i-r_0}.
\]
Notice that the variance of Fairness has similar form with the variance of a linear function that we studied in \secref{LinFun},
where $w_j=S(c_j,c_0)$. If $k_i=\sum{c_j\in C_i}S(c_j,c_0)$, then
\[
\Var{F(c_0)}=\sum_{t_i\in T}k_i^2\Var{X_i}-r_0\sum_{t_i\in T}k_i.
\]
If we clean a tuple $t_i$ then $\Var{X_i}=0$, otherwise we have to consider its variance in the objective function.
$k_i$ is a real number, and hence the problem can be mapped to problem $P_1$ in \secref{LinFun}.
The results follow from Theorems \ref{Th1}, \ref{Th2}.


\subsection{Reduce Uncertainty on Uniqueness}
In this subsection we choose a subset of tuples to clean to minimize the variance on  Uniqueness. Specifically, we aim in finding $A\subseteq T$ such that,
\[
\min_{A\subseteq T, \sum_{t_i\in A} b_i\leq b} \Var{U(c_0)\mid \text{ Tuples }A\text{ are cleaned}}
\]
We can write the variance of $U(c_0)$ as,
\begin{align*}
\Var{U(c_0)}&=\frac{1}{\cardin{C}^2}\Var{\sum_{1\leq j\leq m} \mathbbm{1}(V(c_j,c_0)<0)}=
\frac{1}{\cardin{C}^2}\Var{\sum_{1\leq j\leq m} \mathbbm{1}(\sum_{t_i\in c_j} X_i<w\cdot r_0)}\\
& = \frac{1}{\cardin{C}^2}\left( \sum_{1\leq j\leq m} \Var{\mathbbm{1}(\sum_{t_i\in c_j} X_i<w\cdot r_0)} + 2\sum_{j\neq l}\CoVar{\mathbbm{1}(\sum_{t_i\in c_j}
X_i<w\cdot r_0), \mathbbm{1}(\sum_{t_i\in c_l} X_i<w\cdot r_0)}\right)
\end{align*}
The variance of Uniqueness has the same form with the the sum of Indicator Functions, so all the results in \secref{SIF} can be used
to reduce the uncertainty on Uniqueness.

\subsection{Reduce Uncertainty on Robustness}
To minimize the variance on robustness we use the same technique for Uniqueness. The reason is that those two measures are not so different.
First note that w.l.o.g. we can skip the factor $e$ and keep only the exponent. In addition, the factor $\min\{0,V(c_j,c_0)\}$ can be written
as $V(c_j,c_0)\cdot \mathbbm{1}(V(c_j,c_0)<0)$. The only difference with the Uniqueness measurement is that $V(c_j,c_0)\cdot \mathbbm{1}(V(c_j,c_0)<0)$
is a discrete random distribution, while $\mathbbm{1}(V(c_j,c_0)<0)$ is a bernoulli distribution. All the results from \secref{SIF}, can be used for Robustness
as well, so we can have an efficient constant approximation from minimizing the variance on the robustness of a claim.


\subsection{Reduce Uncertainty on Counter Claims}
In this section, given a claim $c_0$, the goal is to clean a set of tuples $A\subseteq T$ to maximize the probability that a good counter claim of $c_0$ exists
in the set of claims $C$. Recall, that a claim $c_j$ is a good counter claim of $c_0$ if $V(c_j,c_0)$ is a small negative value and $S(c_j,c_0)$ is large.
More specifically, in order to define the optimization problem, we clean a set of tuples to maximize the probability that a good counter claim, \emph{in average},
exists. When we choose to clean a tuple $t_i$, then its value is drawn form its random distribution $X_i$. On the other hand, if we choose not to clean the tuple $t_i$ then its value will be equal to the current value $a_i$.

\begin{align*}
&\max_{A\subseteq T: \sum_{t_i\in A}b_i\leq b}\Prob{\sum_{1\leq j\leq m}S(c_j,c_0)\cdot V(c_j,c_0)<0 \mid \text{Tuples }A\text{ are cleaned}}\\
&=\max_{A\subseteq T: \sum_{t_i\in A}b_i\leq b}\Prob{\sum_{t_i\in A}k_iX_i -m\cdot r_0+\sum_{t_i\notin A}k_ia_i<0}\\
&=\max_{A\subseteq T: \sum_{t_i\in A}b_i\leq b}\Prob{\sum_{t_i\in A}k_iX_i+\sum_{t_i\notin A}k_ia_i<m\cdot r_0}.
\end{align*}
If we introduce the binary variable $x_i$, which is $1$ if we clean the tuple $t_i$ and $0$ if we do not clean $t_i$ then we can write the problem with the following way:
\begin{equation*}
\begin{array}{ll@{}ll}
P_1: \text{maximize}  & \displaystyle \Prob{\sum_{t_i\in T}x_ik_iX_i + \sum_{t_i\in T}(1-x_i)k_ia_i < m\cdot r_0} &&\\
\text{subject to}& \displaystyle \sum_{t_i\in T}b_ix_i\leq b,  &\\
                 & x_{i} \in \{0,1\}, i=1 ,..., n & &
\end{array}
\end{equation*}
or equivalently,
\begin{equation*}
\begin{array}{ll@{}ll}
P_2: \text{maximize}  & \displaystyle \Prob{\sum_{t_i\in T}k_i(X_i-a_i)x_i < m\cdot r_0 - \sum_{t_i\in T}k_ia_i} &&\\
\text{subject to}& \displaystyle \sum_{t_i\in T}b_ix_i\leq b,  &\\
                 & x_{i} \in \{0,1\}, i=1 ,..., n & &
\end{array}
\end{equation*}
Notice that $P_2$ has the same form with $P_p$ and hence the results of \secref{MaxProb} can be used to get exact an exact pseudo-polynomial
algorithm if $X_i$'s are normal distributions.
Notice that, intuitively, the current value $a_i$ can be equal to the expectation of the random variable $X_i$
(if we do not clean a tuple $t_i$ then we consider its value to be equal to the expectation $\Expec{X}$).
It is known that if $X_i$ is normal distribution
then $X_i-a_i$ for real $a_i$'s is also a normal distribution. Furthermore, $\Expec{X_i-a_i}=\Expec{X_i}-a_i=0$ if $a_i=\Expec{X_i}$.
In \secref{MaxProb} we assumed that $\Expec{D_i}=0$ in order to derive a constant approximation algorithm. For finding counter claims, if we set $D_i=X_i-a_i$
then $\Expec{D_i}=0$ and hence the approximation algorithm holds. 

==> maxprob.tex <==
\section{Maximize Probability}
\seclab{MaxProb}
The goal of this section  is to clean a set of tuples $T\subseteq \PntSet$,
with $\sum_{\pnt_i\in T}b_i\leq b$ to maximize the probability that $\Prob{f(\cdot)<0}$ where $f$ is a linear function.
Let $f(D_{S_1},\ldots, D_{S_m}, r) = \sum_{1\leq j\leq m}w_jD_{S_j} +w_{j+1}r=\sum_{1\leq i\leq n}k_iD_i + w_{j+1}r$, for $w_j\in \Re$.
In this section we consider that the random variables $D_j$ may take negative values as well.
The problem can be written as,
\[
P_p: \max_{T\subseteq \PntSet, \sum_{\pnt_i\in T}b_i\leq b}\Prob{\sum_{\pnt_i\in T}k_iD_i +w_{j+1}r\geq 0}
\]
The objective of $P_p$ is $\Prob{\sum_{\pnt_i\in T}k_iD_i\geq -w_{j+1}r}$.
Notice that if $-w_{j+1}r\leq 0$ then problem $P_p$ is trivial because for $T=\emptyset$,
$\Prob{0\geq -w_{j+1}r}=1$. Next, we assume that $-w_{j+1}r=\phi>0$.

Before we study problem $P_p$ let us mention an easier version  of the problem, minimize the expectation of $f(\cdot)$.
Namely,
\[
P_E: \max_{T\subseteq \PntSet, \sum_{\pnt_i\in T}b_i\leq b}\Expec{\sum_{\pnt_i\in T}w_iD_i +w_{j+1}r}
\]
Because of the linearity of expectation we have $\Expec{\sum_{\pnt_i\in T}k_iD_i +w_{j+1}r}=\sum_{\pnt_i\in T}k_i\Expec{D_i} +w_{j+1}r$.
If we skip all terms with $k_i\Expec{D_i}\leq 0$, the problem can be mapped to the Knapsack problem and solved exactly in pseudo-polynomial time
or approximately in polynomial time.

Back to $P_p$ problem, unfortunately the problem is not as easy as $P_E$. Notice that the probability depends on the variance of $f(\cdot)$, except of
its expectation. Problem $P_p$ is a probabilistic linear program and generally those problems are hard due to the non-convexity. Later we show, some of the
known results and some approximation that we can get for Normal Distributions.

Notice that Problem $P_p$ has a unique constraint and it seems like a Knapsack problem.
In particular, it is an instance of Probabilistic $0/1$ Knapsack problem with stochastic rewards
as it has been defined in \cite{steinberg1979preference} and in a series of other papers. In most of these papers
they tackle the program using Dynamic Programming or writing the problem as an Integer constraint
problem. In the worst case, the algorithms need to solve an exponential number of subproblems
to gen the optimum solution.

Next, we concentrate on Normal distributions. In \cite{morton1998stochastic} they
propose a pseudo-polynomial algorithm, as a generalization from Knapsack problem with
multiple constraints, for problem $P_p$ if variables $D_i$ are normal
distributions.
In our case, we propose a simpler exact pseudo-polynomial algorithm and a fully polynomial approximation
algorithm making the assumption that $\Expec{D_i}=0$ for all $1\leq i\leq n$. As we will see in the next section,
this assumption is reasonable for some real problems on cleaning data.

Let $D_i$ be a normal distribution with $\Expec{D_i}=0$ and $\Var{D_i}$. Let
$\mathcal{N}(0,1)$ denote the standard normal distribution.
Following the analysis of \cite{morton1998stochastic}, we can write our objective as
\begin{align*}
 \Prob{\sum_{\pnt_i\in T} k_i\cdot D_i\geq \phi} &= \Prob{\sum_{\pnt_i\in T} k_i\cdot \Expec{D_i}+ \mathcal{N}(0,1)\sqrt{\sum_{\pnt_i\in T} k_i^2\cdot \Var{D_i}}\geq \phi}\\
						&= \Prob{\mathcal{N}(0,1)\sqrt{\sum_{\pnt_i\in T} k_i^2\cdot \Var{D_i}}\geq \phi}\\
						&= \Prob{\mathcal{N}(0,1)\geq \frac{\phi}{\sqrt{\sum_{\pnt_i\in T} k_i^2\cdot \Var{D_i}}}}
\end{align*}
The maximum probability above is taken when the quantity $\frac{\phi}{\sqrt{\sum_{\pnt_i\in T} k_i^2\cdot \Var{D_i}}}$
is minimized. So the optimum subset to clean is the same with
the optimum subset of the following problem:
\[
\hat{P}_p: \max_{T\subseteq \PntSet, \sum_{\pnt_i\in T}b_i\leq b}\sum_{\pnt_i\in T}k_i^2\cdot \Var{D_i}
\]
Problem $\hat{P}_p$ is an instance of the Knapsack problem, so using
the exact dynamic pseudo-polynomial algorithm we can get an exact solution for $P_p$.
Intuitively, it says that if all $D_i$'s have mean equals to $0$,
then we should choose to clean objects with high variance and small cost in order to
maximize the probability that $\sum_{\pnt_i\in T}k_iD_i\geq \phi$.
\begin{theorem}
If $\Expec{D_i}=0$ for $1\leq i\leq n$, there is an optimal algorithm for problem $P_p$ that runs in time $O(n^2b)$ (or $O(nb)$ if costs $b_i$ are integers).
\end{theorem}

\paragraph{Approximation}
Since $\hat{P}_p$ is an instance of the Knapsack problem, we can get an FPTAS.
If $OPT$ is the optimum solution for $\hat{P}_p$, then we can get a solution with
value $ALG$ in polynomial time, such that $ALG\geq (1-\epsilon)OPT$. By doing simple
calculations we have $\frac{\phi}{\sqrt{ALG}}\leq \frac{1}{\sqrt{1-\epsilon}}\frac{\phi}{\sqrt{OPT}}$.
Let $OPT' = \frac{\phi}{\sqrt{OPT}}$ and $ALG'=\frac{\phi}{\sqrt{ALG}}$. We assume that
$\epsilon\leq 3/4$ and we have
\[
 ALG'\leq 2\cdot OPT'.
\]
The maximum probability is computed by $\Prob{\mathcal{N}(0,1)\geq OPT'}$.
In our case we have,
\[
 \Prob{\mathcal{N}(0,1)\geq ALG'}\geq \Prob{\mathcal{N}(0,1)\geq 2\cdot OPT'}
\]
The overall approximation error would be the value of the minimum ratio
\[
\frac{\Prob{\mathcal{N}(0,1)\geq 2\cdot OPT'}}{\Prob{\mathcal{N}(0,1)\geq OPT'}}=
\frac{\int_{2\cdot OPT'}^{\infty}e^{-\frac{1}{2}t} \diff t}{\int_{OPT'}^{\infty}e^{-\frac{1}{2}t} \diff t}
\]
Unfortunately, the function $\frac{\int_{2\cdot OPT'}^{\infty}e^{-\frac{1}{2}t} \diff t}{\int_{OPT'}^{\infty}e^{-\frac{1}{2}t} \diff t}$
is decreasing for $x\geq 0$ and
$\lim_{x\rightarrow \infty}\frac{\int_{2x}^{\infty}e^{-\frac{1}{2}t} \diff t}{\int_{x}^{\infty}e^{-\frac{1}{2}t} \diff t}=0$,
so the approximation ratio can be arbitrarily small, for very large values of $OPT'$.
Notice that if $OPT'$ is large, then $\Prob{\mathcal{N}(0,1)\geq OPT'}$
is very small. For example, even if $OPT'=4$, then $\Prob{\mathcal{N}(0,1)\geq OPT'}=0.00003$.
In these cases it is usual to consider that there is a lower bound
on the minimum possible probability.
%For example, in \cite{henig1990risk} they show an algorithm
%for $P_2^*$ for normal distributions that find the optimum solution efficiently
%when the objective maximum probability is greater than $1/2$.
In practice if the maximum probability is very small then we can consider that it is
zero.
In our case we assume that, if $\Prob{\mathcal{N}(0,1)\geq OPT'}<0.05$
then we can safely consider that the probability is equal to $0$. If we set,
$\Prob{\mathcal{N}(0,1)\geq OPT'} = \int_{OPT'}^{\infty}e^{-\frac{1}{2}t} \diff t= 0.05$ then
we find $OPT'\approx 1.64$, and so we assume that $OPT'\leq 1.64$ in order not to have a $0$
probability. The worst approximation ratio will be:
\[
 \frac{\int_{2\cdot 1.64}^{\infty}e^{-\frac{1}{2}t} \diff t}{\int_{1.64}^{\infty}e^{-\frac{1}{2}t} \diff t} \geq 1/100=O(1).
\]
So we can conclude,
\begin{theorem}
If $\Expec{D_i}=0$ for $1\leq i\leq n$, there is an algorithm that runs in $O(\frac{n^3}{\epsilon})$ time (or $O(\frac{n^2}{\epsilon})$ if costs $b_i$ are integers),
and if $OPT>0.05$, it finds a value $A$ such that $A= O(OPT)$.
\end{theorem}

==> minvar.tex <==
\section{Minimize Variance}
\seclab{MinVr}

In this section we study the problem of choosing a subset of objects to clean
to minimize the variance of function $f(\cdot)$. First we study the easier
case where $f(\cdot)$ is a linear function, and later we consider the more
complicated sum of Indicator Functions.

\subsection{Linear Function}
\seclab{LinFun}
Let $f(D_{S_1}, \ldots, D_{S_m}, r)=\sum_{1\leq j\leq m}w_jD_{S_{j}} + w_{m+1}r$, where $w_j\in \Re$.
Since $w_{m+1}r$ is a real number we can skip it from our computations. The function that we want to minimize
is $\Var{\sum_{1\leq j\leq m}w_jD_{S_{j}}}$. If $C_i=\{S_j\mid \pnt_i\in S_j\}$, we have,
\[
\Var{\sum_{1\leq j\leq m}w_jD_{S_{j}}} = \Var{\sum_{1\leq j\leq m}w_j\sum_{\pnt_i\in S_j}D_i}
=\Var{\sum_{\pnt_i\in S_j}\sum_{1\leq j\leq m}w_j\cdot D_i}
=\Var{\sum_{\pnt_i\in \PntSet}\left(\sum_{S_j\in C_i}w_j\right) D_i}.
\]
For simplicity, let $k_i=\sum_{S_j\in C_i}w_j$. Thus, we can write,
\[
\Var{\sum_{\pnt_i\in \PntSet}k_i\cdot D_i} = \sum_{\pnt_i\in \PntSet}k_i^2\cdot \Var{D_i}
\]

We define the optimization problem by introducing the binary variables $x_i$, for $1\leq i\leq n$.
$x_i$ takes the value $1$ if we clean the object $\pnt_i$ and the value $0$ if we do not choose
to clean $\pnt_i$. The optimization problem to minimize the variance can be written as follows:
\begin{equation*}
\begin{array}{ll@{}ll}
P_1: \text{minimize}  & \displaystyle \sum_{\pnt_i\in \PntSet}k_i^2\Var{D_i}(1-x_i)&&\\
\text{subject to}
		 &\sum\limits_{\pnt_i\in \PntSet}b_ix_i\leq b &\\
                 & x_{i} \in \{0,1\}, i=1 ,..., n & &
\end{array}
\end{equation*}
Notice that by introducing a variable $y_i=1-x_i$, $P_1$ is similar to the Knapsack minimization problem and known exact pseudo-polynomial algorithms,
approximation fully polynomial algorithms are known.

By writing the objective function as
$\min \sum_{\pnt_i\in \PntSet}k_i^2\Var{D_i}(1-x_i) = \sum_{\pnt_i\in \PntSet}k_i^2\Var{D_i}-\max\sum_{\pnt_i\in \PntSet}k_i^2\Var{D_i}x_i$,
we can write $P_1$ as a maximization Knapsack problem:
\begin{equation*}
\begin{array}{ll@{}ll}
P'_1: \text{maximize}  & \displaystyle \sum_{\pnt_i\in \PntSet}k_i^2\Var{D_i}x_i&&\\
\text{subject to}
		 &\sum\limits_{\pnt_i\in \PntSet}b_ix_i\leq b &\\
                 & x_{i} \in \{0,1\}, i=1 ,..., n & &
\end{array}
\end{equation*}
In order to use known algorithms for the different versions of Knapsack problems
we first need to compute the variances $\Var{D_i}$ for all $1\leq i\leq n$.
It is straightforward to compute all of them in $O(qn)$ time.
So we conclude to the next theorems:
\begin{theorem}
\label{Th1}
 Let $\PntSet$ be a set of $n$ objects associated with uncertainty, and
 $m$ sets $S_j\subseteq\PntSet$ as defined above. Given a budget $b$, the optimum set of objects
 to clean to minimize the variance over a linear function $f(D_{S_1},\ldots, D_{S_m})$
 can be found in $O((b+q)n)$ time.
\end{theorem}

\begin{theorem}
\label{Th2}
 Let $\PntSet$ be a set of $n$ objects associated with uncertainty, a parameter $\epsilon>0$, and
 $m$ sets $S_j\subseteq\PntSet$ as defined above. Given a budget $b$, a set $T\subseteq \PntSet$
 can be found in $O(n^3/\epsilon)$ such that $\Var{f(D_{S_1},\ldots, D_{S_m})\mid \text{ Clean tuples } T}\leq (1+\epsilon)V_{OPT}$,
 where $V_{OPT}$ is the minimum uncertainty.
\end{theorem}

\subsection{Sum of Indicator Functions}
\seclab{SIF}
In this subsection we study the case where $f(\cdot)$ is a sum over Indicator Functions,
namely,
\[
f = \sum_{1\leq j\leq m} \mathbbm{1}(D_{S_j}<r)=\sum_{1\leq j\leq m}\mathbbm{1}(\sum_{\pnt_i\in S_j}D_i<r).
\]
For simplicity we assume that $S_j\cap S_l=\emptyset$ for all $j\neq l$, .i.e. $D_{S_j}$ is independent of $D_{S_l}$.
Later, we remove that assumption.

The goal is to minimize the variance which can be written as
\[
\Var{\sum_{1\leq j\leq m}\mathbbm{1}(\sum_{\pnt_i\in S_j}D_i<r)} = \sum_{1\leq j\leq m}\Var{\mathbbm{1}(\sum_{\pnt_i\in S_j}D_i<r)},
\]
by our assumption that $S_j\cap S_l = \emptyset$. Notice that the random variable $\mathbbm{1}(\sum_{\pnt_i\in S_j}D_i<r)$
is a Bernoulli random variable with success probability $\Prob{\sum_{\pnt_i\in S_j}D_i<r}$ and variance
$\Prob{\sum_{\pnt_i\in S_j}D_i<r}(1-\Prob{\sum_{\pnt_i\in S_j}D_i<r})$.

\paragraph{Non Decreasing Uncertainty}
In contrast to the Linear functions, for an indicator function if we clean an object
we may increase the variance and not decrease it.
The intuition is that the variance of a function $\mathbbm{1}(\sum_{\pnt_i\in S_j}D_i<r)$
depends on the condition $\sum_{\pnt_i\in S_j}D_i<r$. If we clean the value of $D_z$, say $D_z=x_z$
the condition $\sum_{\pnt_i\in S_j\setminus\{\pnt_z\}}D_i+x_z<r$ may become either harder or easier to satisfy.
It seems to be an issue since in that case variance is not monotonically decreasing. To see
why this is true let see a simple example. Suppose that $r=3$ and objects
$\pnt_1, \pnt_2, \pnt_3$ with Bernoulli random variables $D_1, D_2, D_3$
and success probabilities $1/2, 1/3, 1/4$, respectively. Furthermore,
let $S_1=\{\pnt_1, \pnt_2,\pnt_3\}$ be the unique set of points.
Initially, the variance is
$\Prob{D_1+ D_2+ D_3<3}(1-\Prob{D_1+D_2+D_3<3})=23/(24)^2=0.0399$.
Let clean the object $\pnt_1$. There are two cases:
\begin{itemize}
\item If $D_1=0$, $Pr[D_2+D_3<3]=1$, so the uncertainty now is $0$ (decreased). On the other hand,
\item If $D_1=1$, then $Pr[D_2+D_3< 2]=11/12$ and $Pr[D_2+D_3<2](1-Pr[D_2+D_3<2])=11/(12)^2=0.0763>0.0399$. In this case the uncertainty increased after cleaning $\pnt_1$.
\end{itemize}


\paragraph{Expected Uncertainty}
We would like to have a decreasing measure of the uncertainty.
In this section we define the notion of the \emph{Expected Uncertainty}, denoted by $EU$.
Briefly, given a set $T$ of objects to clean, $EU(T,\PntSet)$ is the expected variance
of function $f(\cdot)$ after cleaning objects $T\subseteq \PntSet$. If $\PntSet$ is clear from the context we use $EU(T)=EU(T,\PntSet)$.
Relevant quantities have been defined in other works, \cite{cheng2008cleaning, mo2013cleaning}.
In order to define exactly the expected uncertainty we first need to introduce some notation.
Given a set of objects $T\subseteq \PntSet$, all possible realizations of the objects in $T$
are denoted by $R_T$. For a realization $\rea\in R_T$, let $\rea_i$ be the realization of variable
$D_i$, and $M_{\rea,S_j}=\sum_{\pnt_i\in T\cap S_j}\rea_i$. In order to simplify the notation let
$V(T,S_j,\rea)=\Prob{\sum_{\pnt_i\in S_j\setminus T}D_i<r-M_{\rea,S_j}}(1-\Prob{\sum_{\pnt_i\in S_j\setminus T}D_i<r-M_{\rea,S_j}})$.
Given a set of objects $T\subseteq\PntSet$ to clean, the expected uncertainty is defined as:
\[
EU(T,\PntSet)= \sum_{\rea\in R_T}\Prob{\bigcap_{\pnt_i\in T}D_i=\rea_i}\sum_{1\leq j\leq m}V(T,S_j,\rea) = \sum_{\rea\in R_T}\left(\prod_{\pnt_i\in T}\Prob{D_i=\rea_i}\right)\sum_{1\leq j\leq m}V(T,S_j,\rea).
\]

Now we can redefine our problem in terms of the expected uncertainty.
\[
 P: \min_{T\subseteq \PntSet, \sum_{\pnt_i\in T}b_i\leq b}EU(T)
\]
We can show the following Lemmas.
\begin{lemma}
\label{Lem1}
 The function $EU$ is decreasing, i.e. for $T_A\subseteq T_B$, $EU(T_A)\geq EU(T_B)$.
\end{lemma}

\begin{lemma}
\label{Lem2}
  The function $EU$ is submodular, i.e. for $T_A\subset T_B$ and $\pnt_i\notin T_B$,
  $EU(T_A\cup \pnt_i)-EU(T_A) \geq EU(T_B\cup \pnt_j)-EU(T_B)$
\end{lemma}
From Lemmas \ref{Lem1}, \ref{Lem2} problem $P$ can be seen as a problem of
minimizing a submodular function with an upper bound constraint.
This is known to be a $NP$-hard problem. Furthermore, let $(\rho,\sigma)$-approximation
of problem $P$ for $\rho\geq 1$ and $0< \sigma\leq 1$, be an algorithm that returns a subset $T\subseteq\PntSet$ of
$\sum_{\pnt_i\in T}b_i\leq \frac{b}{\sigma}$ and $EU(T)\leq \rho EU(T^*)$ where $T^*$ is the optimum set of tuples to clean.
In \cite{svitkina2011submodular} the authors show that there is no $(\rho,\sigma)$-approximation with $\frac{\rho}{\sigma}=o(\sqrt{\frac{n}{\ln n}})$
for the problem of minimizing a submodular function with a cardinality constraint.

Before we mention the known approximation algorithms and what techniques we can use to solve $P$,
we concentrate on a different formulation of our problem.
We define $\bar{EU}(T)=EU(\PntSet\setminus T)$ for $T\subseteq \PntSet$.
We can show that:
\begin{lemma}
\label{Lem3}
  The function $\bar{EU}$ is decreasing and submodular.
\end{lemma}
Let $B$ be the sum of all objects' costs, i.e., $B=\sum_{\pnt_i\in \PntSet}b_i$.
We define the problem
\[
 P': \min_{T\subseteq \PntSet, \sum_{\pnt_i\in T}b_i\geq B-b}\bar{EU}(T)
\]
We can easily observe that
 \[
  (P): \min_{T\subseteq\PntSet, \sum_{\pnt_i\in T}b_i\leq b}EU(T) \Leftrightarrow (P'): \min_{T\subseteq \PntSet,\sum_{\pnt_i\in T}b_i\geq B-b}\bar{EU}(T),
 \]
and
\begin{corollary}
\label{cor2}
 If $OPT_P$, $OPT_{P'}$ is the optimum value of $(P)$ and $(P')$ respectively,
 then $OPT_P=OPT_{P'}$ and any algorithm $A$ that finds a solution of $P'$ with value $A_{P'}$ such that
 $A_{P'}\leq C\cdot OPT_{P'}$ and runs in $O(A_t)$ time, can be used to find a solution of $(P)$ with value $B_P$
 such that $B_P\leq C\cdot OPT_P$ in $O(A_t+n)$ time.
\end{corollary}

\paragraph{Algorithms for $P$ and $P'$}
We show that there exists a $(\frac{1}{\alpha},\frac{1}{1-\alpha})$-approximation for $P$ for any $0<\alpha<1$, a $(5\sqrt{\frac{n}{\ln n}}, \frac{1}{2})$-approximation for $P'$,
and a $(O(\frac{1}{1-k_q}),1)$-approximation for both $P$ and $P'$, where $k_q$ is a real parameter derived of the objective function.

If all costs are uniform, for example all costs are $1$, and the goal is to clean a subset
$T\subseteq \PntSet$ with $\cardin{T}\leq b$, then in \cite{svitkina2011submodular} they
showed a $(5\sqrt{\frac{n}{\ln n}}, \frac{1}{2})$-approximation algorithm for $P'$.
Because of the bicriteria approximation it is not possible to use the same algorithm to solve $P$.
Notice that if $\sum_{\pnt_i\in T}b_i\geq \frac{n-b}{2}$, where $T$ is the solution of $P'$ found by the approximation
algorithm in \cite{svitkina2011submodular}, then $n-\sum_{\pnt_i\in T}b_i \leq \frac{n+b}{2}>> b$ in the worst case.

In order to approximate $P$, we can use techniques described in \cite{svitkina2011submodular, hayrapetyan2005unbalanced}
and give a $(\frac{1}{\alpha},\frac{1}{1-\alpha})$-approximation for $P$ for any $0<\alpha<1$. The general idea is
to formulate the value of a submodular function with a minimum weighted cut in a graph and then using the algorithms
proposed in \cite{hayrapetyan2005unbalanced} to approximate the minimum cut.

Finally, another approximation algorithm is described in \cite{iyer2013submodular} that works for both
$P$, $P'$ and it does not violate the constraint $\sum_{1\leq i\leq n}b_ix_i\leq b$.
They propose an approximation algorithm for the following type of problem:
\[
P_I: \min_{X: g(X)\geq b}q(X)
\]
for submodular functions $g, q$.
Problem $P_I$ is related to $P'$: We can map $q(T)=\bar{EU}(T)$, and $g(T)=\sum_{\pnt_i\in T}b_i$ since $\bar{EU}$ is submodular and the sum
$\sum_{\pnt_i\in T}b_i$ is a (sub)modular function.
As a result, $P'$ can be solved using
the techniques in \cite{iyer2013submodular}. They propose a $(O(\frac{1}{1-k_q}H_q), 1)$-approximation algorithm
for the problem, where $k_q=1-\min_{\pnt_i\in\PntSet}\frac{q(\PntSet)-q(\PntSet\setminus\{\pnt_i\}}{q(\pnt_i)}$
is the curvature of function $q$ and intuitively measures the distance from $q$ from modularity.
If $k_q=1$, then the approximation ratio becomes $(O(\sqrt{n\log n}H_q), 1)$. The parameter $H_q$
is the approximation ratio of problem $P_I$ assuming that $q$ is modular.
To find $H_q$ in our setting, notice that $g$ is also modular and hence we solve $P_I$ assuming that both $q, g$ are modular functions.
There are different techniques to solve $P_I$ with modular functions:
\begin{itemize}
  \item Using the result in \cite{wolsey1982analysis} we can get a $H_q=O(\log n)$-approximation.
  \item Problem $P_I$ can be solved as a Knapsack problem. If costs are integers we can get a pseudo-polynomial exact algorithm, and hence $H_q=1$.
  \item Even if costs are not integers there is an FPTAS for the Knapsack problem so we can get a $H_q=(1+\epsilon)$-approximation ratio in polynomial time.
\end{itemize}
Using the above results we can get a $(O(\frac{1}{1-k_q}),1)$-approximation for $P_I$, if $k_q\neq 1$, or a
$(O(\sqrt{n\log n}), 1)$-approximation if $k_q=1$. This algorithm solves $P'$, but as we showed
from Corollary~\ref{cor2} the approximation algorithm works for problem $P$, as well.

\begin{theorem}
\label{Th:Uniq}
There are approximation algorithms, with approximation ratio $(\frac{1}{\alpha},\frac{1}{1-\alpha})$ for any $0<\alpha<1$, or approximation
ratio $(O(\frac{1}{1-k_q}),1)$ that run in polynomial time for problem $P$.
\end{theorem}

If we remove the assumption that $S_j\cap S_l=\emptyset$ for all $j\neq l$ then $D_{S_j}, D_{S_l}$ are not independent.
In this case we have,
\[
\Var{\sum_{1\leq j\leq m}\mathbbm{1}(\sum_{\pnt_i\in S_j}D_i<r)} = \sum_{1\leq j\leq m}\Var{\mathbbm{1}(\sum_{\pnt_i\in S_j}D_i<r)}+
2\sum_{j\neq l}\CoVar{\left(\mathbbm{1}(\sum_{\pnt_i\in S_j}D_i<r)\right), \left(\mathbbm{1}(\sum_{\pnt_i\in S_l}D_i<r)\right)},
\]
where $\CoVar{X,Y}$ denotes the covariance of variables $X, Y$.
Using the equality $\CoVar{X,Y}=\Expec{XY}-\Expec{X}\Expec{Y}$, We define the expected uncertainty as a function of variance, covariance:
\begin{align*}
EU(T,\PntSet) & = \sum_{\rea\in R_T}\left(\prod_{\pnt_i\in T}\Prob{D_i=\rea_i}\right) \sum_{1\leq j\leq m}V(T,S_j,\rea)\\
& +2\sum_{j\neq l}\Expec{\mathbbm{1}(\sum_{\pnt_i\in S_j\setminus T}D_i<r-M_{\rea,S_j})\cdot \mathbbm{1}(\sum_{\pnt_i\in S_l\setminus T}D_i<r-M_{\rea,S_l})}\\
& \qquad -2\Expec{\mathbbm{1}(\sum_{\pnt_i\in S_j\setminus T}D_i<r-M_{\rea,S_j})}\cdot \Expec{\mathbbm{1}(\sum_{\pnt_i\in S_l\setminus T}D_i<r-M_{\rea,S_l})}.
\end{align*}
We know that $V(T,S_j,\rea)= \Prob{\sum_{\pnt_i\in S_j\setminus T}D_i<r-M_{\rea,S_j}}(1-\Prob{\sum_{\pnt_i\in S_j\setminus T}D_i<r-M_{\rea,S_j}})$ and\\ $\Expec{\mathbbm{1}(\sum_{\pnt_i\in S_j\setminus T}D_i<r-M_{\rea,S_j})}= \Prob{\sum_{\pnt_i\in S_j\setminus T}D_i<r-M_{\rea,S_j}}$.
Skipping the details and based on the proof of Lemmas \ref{Lem1}, \ref{Lem2} we can show that that $EU$ is a decreasing and submodular function,
and hence the results of Theorem \ref{Th:Uniq} still holds.


==> more-model.tex <==
Note that one can use tail probabilities (instead of variance) as a
measure of uncertainty.  Therefore, the problem of minimizing
uncertainty can be alternatively defined as follows:
\begin{equation}
  \begin{split}
    \text{minimize:}\;%
    & \sum_{\mathbf{v} \in V_T}%
    \Prob{\forall \obj_i \in T: X_i = v_i} \cdot%
    \Prob{f(\mathbf{X}) < \tau \mid \forall \obj_i \in T: X_i = v_i}\\
    \text{subject to:}\;%
    & \sum_{\obj_i \in T} c_i \le C.
  \end{split}
\end{equation}
But the above problem remains different from maximizing surprise.  For
a clearer comparison, we rewrite the objective function for maximizing
surprise as follows:
\begin{equation}
  \begin{split}
    \text{maximize:}\;%
    & \sum_{\mathbf{v} \in V_T}%
    \Prob{\forall \obj_i \in T: X_i = v_i} \cdot%
    \One{f(\mathbf{X}) < \tau \mid%
      \forall \obj_i \in T: X_i = v_i;\;%
      \forall \obj_i \in \Objs \setminus T: X_i = u_i
    }\\
    \text{subject to:}\;%
    & \sum_{\obj_i \in T} c_i \le C.
  \end{split}
\end{equation}
Note that the $\One{\cdot}$ term in the objective function above is
deterministic---all $X_i$ variable is assigned a concrete value.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:


==> proofs3.tex <==
\begin{proof} (of Lemma~\ref{lemma:linear-modular})
Since the components of $\*X$ are pairwise uncorrelated we have $\Cov{a_iX_i, a_jX_j}=0$ for all $i \neq j$.
We show that $\Var{f(\*X) \mid \*X_T = \*v}=\sum_{\obj_i \in \Objs \setminus T} a_i^2 \Var{X_i}$, hence, minimizing
$\sum_{\*v \in \*V_T} \Prob{\*X_T = \*v} \cdot \Var{f(\*X) \mid \*X_T = \*v}$ is the same as minimizing
$\sum_{\obj_i \in \Objs \setminus T} a_i^2 \Var{X_i}$. Equivalently we can write the problem as minimizing
$\sum_{\obj_i \in T'} a_i^2 \Var{X_i}$ such that\\$\sum_{\obj_i\in T'}c_i\geq \sum_{\obj_i\in \Objs}c_i-C$. The result follows.

In order to show the second part of the lemma we note that if $\*X_{\Objs \setminus T} = \*u_{\Objs \setminus T}$,
then $f(\*X) - f(\*u)=\*a_T ( \*X_T - \*u_T )$.
Since $X_i \sim N(u_i, \sigma_i^2)$ and all $X_i$'s are independent,
  $f(\*X) - f(\*u) \sim N(0, \sum_{\obj_i \in T} a_i^2 \sigma_i^2)$.
Therefore, we can show that\\
$\Prob{f(\*X) < f(\*u) - \tau \mid \*X_{\Objs \setminus T}}=\Prob{N(0, 1) < {-\tau \over \sqrt{\sum_{\obj_i \in T} a_i^2 \sigma_i^2}}}$.
Maximizing the above is equivalent to maximizing
$\sum_{\obj_i \in T} a_i^2 \sigma_i^2$, so the objective is additive with $w_i = a_i^2 \sigma_i^2$.
\end{proof}

\begin{proof} (of Lemma~\ref{corollary:modular-maxpr})
From Lemma~\ref{lemma:linear-modular} we can formulate the \MaxPr\ problem as
$\max_{T\subseteq \Objs, \sum_{\obj_i\in T} c_i\leq C}\Prob{\sum_{\obj_i\in T}a_iX_i< -\tau}$,
where $a_i$ are real numbers and $\tau$ is a positive number.
Following the analysis of \cite{morton1998stochastic} we can conclude that
$\Prob{\sum_{\obj_i\in T}a_iX_i< -\tau}=\Prob{\mathcal{N}(0,1)< \frac{-\tau}{\sqrt{\sum_{\obj_i\in T} a_i^2\cdot \Var{X_i}}}}$.
So the optimum subset to clean is the same with the optimum subset of the following problem:
$\max_{T\subseteq \Objs, \sum_{\obj_i\in T}c_i\leq C}\sum_{\obj_i\in T}a_i^2\cdot \Var{X_i}$, which is an instance of the maximum Knapsack problem,
so using the exact dynamic pseudo-polynomial algorithm we can get an exact solution.

For the second part of the lemma we use an FPTAS for maximum Knapsack problem we defined above.
If $P^*$ is the value of the optimum solution for that Knapsack problem we set $P'=\frac{-\tau}{\sqrt{P^*}}$.
Using the cumulative function of the normal distribution and the FPTAS solution we get an algorithm with approximation factor
$\frac{\Prob{\mathcal{N}(0,1)< 2\cdot P'}}{\Prob{\mathcal{N}(0,1)< P'}}=
\frac{\int_{2\cdot P'}^{-\infty}e^{-\frac{1}{2}t} \diff t}{\int_{P'}^{-\infty}e^{-\frac{1}{2}t} \diff t}$.
Assuming that $\OPT>0.05$, i.e., $\Prob{\mathcal{N}(0,1)< P'}<0.05$ then $P'\geq -1.64$, which gives an approximation ratio of
$\frac{\int_{2\cdot (-1.64)}^{-\infty}e^{-\frac{1}{2}t} \diff t}{\int_{-1.64}^{-\infty}e^{-\frac{1}{2}t} \diff t} \geq 1/100=O(1)$.
See \cite{fullpaper} for the details of the proof.
\end{proof}

\begin{proof}(of Lemma~\ref{lemma:non-increasing})
We first show an inequality that we use in the current and the next lemma.
Suppose $\sum_{i=1}^n w_i = 1$, and $0 \le w_i \le 1$ for all $1 \le i \le n$. Then, we can show that
 $\left(\sum_{i=1}^n w_ix_i^2\right) - %
    \left(\sum_{i=1}^n w_ix_i\right)^2%
    = \sum_{1 \le i < j \le n} w_iw_j(x_i-x_j)^2%
    \ge 0.$

    Without loss of generality, we assume that
  $T = \{ \obj_1, \obj_2, \ldots, \obj_j \}$ and consider
  $T \cup \{\obj_{j+1}\}$.  For brevity, let $i_1..i_2$ (where
  $1 \le i_1 \le i_2 \le n$) denote
  $\{ \obj_i \mid i_1 \le i \le i_2 \}$, i.e., the set of objects with
  indices between $i_1$ and $i_2$ (inclusive).  Let
  $\concat{\cdot}{\cdot}$ denote the concatenation of (column) vectors
  and/or individual values into a (column) vector.

  We show that,
 \begin{small}
 $\EVar{1..j} - \EVar{1..j+1}=
      \sum_{\*v \in \*V_{1..j}} %
      \Prob{\*X_{1..j} = \*v}\\ (L_1(\*v) - L_0(\*v))$,
      where $L_0(\*v)=
     (\Expected{ f(\*X) \mid \*X_{1..j}=\*v })^2$
 \end{small}
     and
     \begin{small}
     $L_1(\*v)=
     \!\sum_{v_{j+1} \in V_{j+1}}\!\!\!\!\!%
      \Prob{X_{j+1} = v_{j+1} \mid \*X_{1..j} = \*v}\cdot\\
     (\Expected{ f(\*X) \mid \*X_{1..j+1}=\concat{\*v}{v_{j+1}} })^2$.
     \end{small}
     To show that $\EVar{1..j} \geq \\\EVar{1..j+1}$, it suffices to show that
  $\forall \*v \in \*V_{1..j}: L_1(\*v) \ge L_0(\*v)$. We prove that using the inequality we mentioned at the beginning of the proof.
  %The full details of the proof can be found in \cite{fullpaper}.
\end{proof}

The proof of Lemma~\ref{lemma:submodular} is more complicated than the
previous one, however the high level idea is the same.  Using algebra
and the result of the inequality in the previous proof we show that
the objective function of \MinVar\ is submodular.

\begin{proof} (of Lemma~\ref{lemma:Compl})
From the definition, we have that $\EVarComplement{\Objs \setminus \widetilde{T}}=\EVar{\widetilde{T}}$, for any $\widetilde{T}\subseteq \Objs$.
Hence, if $T$ is a solution for the \MinVar\ problem such that $\EVar{T}\leq \alpha \EVar{T^*}$ and $\sum_{\obj_i\in T}c_i\leq C$, where $T^*$ is the optimum set, then $\overline{T}=\Objs\setminus T$ is a solution for the \MinVarComplement\ problem such that $\EVarComplement{\overline{T}} \leq \alpha \EVarComplement{\Objs\setminus T^*}$
and $\sum_{\obj_i\in \overline{T}}c_i\geq \left(\sum_{\obj_i \in \Objs}\right) c_i- C$. From our first observation notice that $\Objs\setminus T^*$ is the optimum set to clean for the \MinVarComplement\ problem.
The same holds in the other direction: An $\alpha$-approximation solution for the \MinVarComplement\ problem is also an $\alpha$-approximation for the \MinVar\ problem. Hence, \MinVar\ problem can be mapped to \MinVarComplement\ problem.

Using the facts that the $\EVar{\cdot}$ function is non-increasing and submodular we can show that $\EVarComplement{\cdot}$ is non-decreasing and submodular.
\end{proof}

\begin{proof} (of Theorem~\ref{th:runtimeDepClaims})
We first consider the Uniqueness ($\duplicity{q^\circ(\*u)}{\*X}$) and later we extend for the Fairness ($\bias{q^\circ(\*u)}{\*X}$) and Robustness ($\fragility{q^\circ(\*u)}{\*X}$).
Let $t$ be an instance of $T$.
We have that $\EVar{T}=\sum_{t\in T}\Prob{t}(\sum_{q\in Q} \Var{\mathbf{1}[\Delta(q, q^\circ) \ge 0] \mid t} + \sum_{q, q'\in Q}\Cov{\mathbf{1}[\Delta(q, q^\circ) \ge 0], \mathbf{1}[\Delta(q', q^\circ) \ge 0] \mid t})$.
Let assume a claim $q\in Q$ and let $T_q$ be the objects in $T\cap (q\cup q^\circ)$.
We observe that $\sum_{t\in T}\Prob{t}\Var{\mathbf{1}[\Delta(q, q^\circ) \ge 0]\mid t}=\sum_{t\in T_q}\Prob{t}\Var{\mathbf{1}[\Delta(q, q^\circ) \ge 0]\mid t}$, since the different values of the tuples that do not belong in $q$ or in $q^\circ$ do not change the variance of $\mathbf{1}[\Delta(q, q^\circ) \ge 0]$. Equivalently, let $q, q'\in Q$ and let $T_{qq'}$ be the objects in $T\cap (q\cup q' \cup q^\circ)$.
We observe that $\sum_{t\in T}\Prob{t}\Cov{\mathbf{1}[\Delta(q, q^\circ) \ge 0],\mathbf{1}[\Delta(q', q^\circ) \ge 0] \mid t} = \sum_{t\in T_{qq'}}\Prob{t}\Cov{\mathbf{1}[\Delta(q, q^\circ) \ge 0],\mathbf{1}[\Delta(q', q^\circ) \ge 0] \mid t}$ since the different values of the tuples that do not belong in $q, q'$, or $q^\circ$ do not change the covariance of $\mathbf{1}[\Delta(q, q^\circ) \ge 0]$ and $\mathbf{1}[\Delta(q', q^\circ) \ge 0]$.

Based on the observations above we can give a polynomial time algorithm to compute the $\EVar{T}$.
We first start computing the variances. For each claim $q\in Q$ we sum over all the instances of $T_q$, which are $O(V^b)$ for a value $b\leq 2W$, since $q, q^\circ$ contain at most $2W$ objects.
For each such instance $t$ it remains to compute $\Var{\mathbf{1}[\Delta(q, q^\circ) \ge 0]\mid t}$. This can be computed in $O(V^{2W-b}W)$ time so in total we need $O(mV^{2W}W)$ to find all the variances of all claims.
Then we continue with computing the covariances.
For a pair of claims $q, q'\in Q$ we sum over all the instances of $T_{qq'}$, which are $O(V^b)$ for a value $b\leq 3W$, since $q, q', q^\circ$ contain at most $3W$ objects.
For each such instance $t$ it remains to compute $\Cov{\mathbf{1}[\Delta(q, q^\circ) \ge 0],\mathbf{1}[\Delta(q', q^\circ) \ge 0] \mid t}$, which can be computed in $O(V^{3W-b}W)$ so in total we need $O(m^2V^{3W}W)$ to find all covariances of all pairs of claims.

If we consider the Robustness then the only difference is that we compute
$\Var{s_k \cdot (\min\{\Delta(q,q^\circ), 0\})^2\mid t}$ and $\Cov{\mathbf{1}[s_k \cdot (\min\{\Delta(q,q^\circ), 0\})^2,s_k \cdot (\min\{\Delta(q',q^\circ), 0\})^2 \mid t}$. The first quantity can be computed in $O(V^{2W}W)$ and the second one in $O(V^{3W}W)$. The same bounds hold for fairness.

Overall, we conclude that the $\EVar{T}$ of $\bias{q^\circ(\*u)}{\*X}$, $\duplicity{q^\circ(\*u)}{\*X}$ and $\fragility{q^\circ(\*u)}{\*X}$
can be computed in $O(m^2V^{3W}W+n)$ time in the worst case.
\end{proof}


\remove{
Instead, using Theorem~\ref{theorem:submodular}, we can get an approximation algorithm
for the \MinVar\ of $\duplicity{q^\circ(\*u)}{\*X}$ and $\fragility{q^\circ(\*u)}{\*X}$
in polynomial time, assuming $\EVar{}$ can also be computed in polynomial time.
In particular, we show that the $\EVar{}$ of $\duplicity{q^\circ(\*u)}{\*X}$ and
$\fragility{q^\circ(\*u)}{\*X}$ can be computed in $O(mLV^{2W}+n)$ time, where $V$ is the maximum support of distributions in $\*X$,
and $L$ is the maximum degree of a claim. The degree of a claim $q\in Q$ is the number of claims that share at least one object with $q$.
The key observation in obtaining this bound is that two claims that do not share any object
can be considered as independent, so the variance in them can be computed efficiently.
We prove the next theorem in \cite{fullpaper}.
\begin{theorem}
\label{th:runtimeDepClaims}
Let $V$ be the maximum support of distributions in $\*X$, $W$ be the window size of the claims, and $L$ be the largest degree of a claim.
For any set $T\subseteq \Objs$, the $\EVar{T}$ of $\duplicity{q^\circ(\*u)}{\*X}$ and $\fragility{q^\circ(\*u)}{\*X}$
can be computed in $O(mLV^{2W}+n)$ time.
\end{theorem}
\remove{
\begin{proof}
We first consider the Uniqueness ($\duplicity{q^\circ(\*u)}{\*X}$) and later we extend for the Robustness ($\fragility{q^\circ(\*u)}{\*X}$).
Let $t$ be an instance of $T$.
We have that $\EVar{T}=\sum_{t\in T}\Prob{t}(\sum_{q\in Q} \Var{\mathbf{1}[\Delta(q, q^\circ) \ge 0] \mid t} + \sum_{q, q'\in Q}\Cov{\mathbf{1}[\Delta(q, q^\circ) \ge 0], \mathbf{1}[\Delta(q', q^\circ) \ge 0] \mid t})$.
Let assume a claim $q\in Q$ and let $T_q$ be the objects in $T\cap q$.
We observe that $\sum_{t\in T}\Prob{t}\Var{\mathbf{1}[\Delta(q, q^\circ) \ge 0]\mid t}=\sum_{t\in T_q}\Prob{t}\Var{\mathbf{1}[\Delta(q, q^\circ) \ge 0]\mid t}$, since the different values of the tuples that do not belong in $q$ do not change the variance of $q$. Equivalently, let $q, q'\in Q$ and let $T_{qq'}$ be the objects in $T\cap (q\cup q')$.
We observe that $\sum_{t\in T}\Prob{t}\Cov{\mathbf{1}[\Delta(q, q^\circ) \ge 0],\mathbf{1}[\Delta(q', q^\circ) \ge 0] \mid t} = \sum_{t\in T_{qq'}}\Prob{t}\Cov{\mathbf{1}[\Delta(q, q^\circ) \ge 0],\mathbf{1}[\Delta(q', q^\circ) \ge 0] \mid t}$ since the different values of the tuples that do not belong in $q, q'$ do not change the covariance of $q, q'$.

Based on the observations above we can give a polynomial time algorithm to compute the $\EVar{T}$.
We first start computing the variances. For each claim $q\in Q$ we sum over all the instances of $T_q$, which are $O(V^b)$ for a value $b\leq W$.
For each such instance $t$ it remains to compute $\Var{\mathbf{1}[\Delta(q, q^\circ) \ge 0]\mid t}$. This can be computed in $O(V^{W-b})$ time so in total we need $O(mV^W)$ to find all the variances of all claims.
Then we continue with computing the covariances.
For a pair of claims that share at least one object $q, q'\in Q$ we sum over all the instances of $T_{qq'}$, which are $O(V^b)$ for a value $b\leq 2W$.
For each such instance $t$ it remains to compute $\Cov{\mathbf{1}[\Delta(q, q^\circ) \ge 0],\mathbf{1}[\Delta(q', q^\circ) \ge 0] \mid t}$, which can be computed in $O(V^{2W-b})$m so in total we need $O(mLV^{2W})$ to find all covariances of all pairs of claims.

If we consider the Robustness then the only difference is that we compute
$\Var{s_k \cdot (\min\{\Delta(q,q^\circ), 0\})^2\mid t}$ and $\Cov{\mathbf{1}[s_k \cdot (\min\{\Delta(q,q^\circ), 0\})^2,s_k \cdot (\min\{\Delta(q',q^\circ), 0\})^2 \mid t}$. The first quantity can be computed in $O(V^W)$ and the second one in $O(V^{2W})$.

Overall, we conclude that the $\EVar{T}$ of $\duplicity{q^\circ(\*u)}{\*X}$ and $\fragility{q^\circ(\*u)}{\*X}$
can be computed in $O(mLV^{2W}+n)$ time in  the worst case.
\end{proof}
}
This running time is polynomial assuming that each claim contains a constant number
of objects (i.e., $W$ is a constant), which is the case in most real applications.\remove{ We note that in \cite{wu2014toward} authors also made the same assumptions.}
%Notice that the running time depends on the dependency between the claims.
%If there are many claims that depend to each other then the running time can be large. On the other hand, if the dependency between the claims is bounded then the %running time is small. In case that the claims are independent the running time becomes $O(mV^W+n)$.
Furthermore, for window aggregate claims, each claim contains $W$ adjacent objects, so each claim has non-zero covariance with at most $O(W)=O(1)$ claims.
In this case the running time can be improved to $O(mV^{2W}+n)$.
}



\remove{
\begin{corollary}
\label{cor:runtimeDepClaims}
Let $V$ be the maximum support of distributions in $\*X$, and let $w$ be the window size of the claims.
For any set $T\subseteq \Objs$, the $\EVar{T}$ of $\duplicity{q^\circ(\*u)}{\*X}$ and $\fragility{q^\circ(\*u)}{\*X}$
for window aggregate claims can be computed in $O(mWV^{2W}+n)$ time.
\end{corollary}
}


\remove{
In particular, we show that the $\EVar{}$ of $\duplicity{q^\circ(\*u)}{\*X}$ and
$\fragility{q^\circ(\*u)}{\*X}$ can be computed in $O(mV^{LW}L^2+n)$ time, where $L$ is the
largest number of claims that an object belongs to, and $V$ is the maximum support of distributions in $\*X$.
The key observation in obtaining this bound is that two claims that do not share any object
can be considered as independent, so the variance in them can be computed efficiently.
We prove the next theorem in \cite{fullpaper}.

%assuming that each claim contains a constant number of objects, as in \cite{wu2014toward}.
%The key observations in order to get this running time are:
%(i) if an object belongs to $L$ claims then each time that a tuple that belongs to one of these claims is selected to clean,
%the $L$ claims depend to each other and hence the $\EVar{\cdot$} can be computed in $O(f^{LW}L^2)$ time.
%(ii) if two claims do not intersect (do not share a tuple) then


%We can show the following theorem, whose proof can be found in Appendix.
%The proof of the next Theorem can be found in the full version of the paper \cite{fullpaper}.
\begin{theorem}
\label{th:runtimeDepClaims}
Let $V$ be the maximum support of distributions in $\*X$, $w$ be the window size of the claims, and $L$ be the largest number of claims that
an object can belong to. For any set $T\subseteq \Objs$, the $\EVar{T}$ of $\duplicity{q^\circ(\*u)}{\*X}$ and $\fragility{q^\circ(\*u)}{\*X}$
can be computed in $O(mV^{LW}L^2+n)$ time.
\end{theorem}
This running time is polynomial assuming that the dependency between the claims
is bounded (i.e., $L$ is constant) and that each claim contains a constant number
of objects (i.e., $W$ is a constant).\remove{ We note that in \cite{wu2014toward} authors also made the same assumptions.}
%Notice that the running time depends on the dependency between the claims.
%If there are many claims that depend to each other then the running time can be large. On the other hand, if the dependency between the claims is bounded then the %running time is small. In case that the claims are independent the running time becomes $O(mV^W+n)$.
Furthermore, for window aggregate claims, $L$ is at most $2W-1$, because claims contain $W$ adjacent objects, so in the worst case the running time would be $O(mW^2V^{2W^2-W}+n)$, polynomial for constant $W$.
}


\begin{proof} (of Theorem~\ref{theorem:minvar-maxpr-equivalence})
If the independence assumption holds then the result follows easily by Lemma~\ref{lemma:linear-modular}.
We can extend the above argument when the independence assumption does not hold.
Using Lemma~\ref{lemma:linear-modular} we can show that the objective of \MinVar\ problem is
$\max_{T\in \subseteq \Objs} \sum_{\obj_i \in T}
      \,\sum_{\obj_j \in  T}
      \Cov{a_iX_i, a_jX_j}$.
For the second part of the lemma, we can show that the objective of \MaxPr\ problem is
 %\underset{\substack{\SubSet \subseteq X \\ \cardin{\SubSet} = k}}{\argmax}
$\underset{T\subseteq \Objs}{\max}\Prob{N(0, 1) <
    {-\tau \over \sqrt{\underset{\obj_i \in T}{\sum}
      \,\underset{\obj_j \in  T}{\sum}
      \Cov{a_iX_i, a_jX_j}}}}$.
Since $\tau>0$, this is equivalent to
$\underset{T\subseteq \Objs}{\max} \underset{\obj_i \in T}{\sum}
      \,\underset{\obj_j \in  T
      }{\sum}
      \Cov{a_iX_i, a_jX_j}$,
and the result follows.
\end{proof}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:


==> tikz/tikzscale/README <==
----------------------------------------------------------------
tikzscale --- Absolute resizing of TikZ pictures and PGF plots without
              scaling text
E-mail: pat_h@web.de Released under the LaTeX Project
Public License v1.3c or later See http://www.latex-project.org/lppl.txt
----------------------------------------------------------------

The tikzscale package extends the includegraphics command to support
tikzpictures. It allows scaling of TikZ images and PGFPlots to a provided
width or height without changing the text size.

Usage: \usepackage{tikzscale}

As an example write
\includegraphics{myTikZFile.tikz}
instead of
\includegraphics{myJPEGFile.jpeg},
with myTikZFile.tikz being the file name of a text file containing
everything from \begin{tikzpicture} to \end{tikzpicture}. To actually
do some scaling of the included TikZ file, give either an absolute width
or an absolute height in the optional argument, e.g.
\tikzscale@includetikz[width=0.5\linewidth]{myTikZFile.tikz}.
If the file contains a plot created with the PGFPlots package, set both
width and height via the optional argument, e.g.
\tikzscale@includetikz[width=\linewidth,height=0.4\linewidth]{myPGFPlot.tikz}.


